Simulating transgenerational hologenomes under selection with RITHMS

A holobiont is made up of a host organism together with its microbiota. In the context of animal breeding, the holobiont can be viewed as the single unit upon which selection operates. Therefore, integrating microbiota data into genomic prediction models may be a promising approach to improve predictions of phenotypic and genetic values. Nevertheless, there is a paucity of hologenomic transgenerational data to address this hypothesis, and thus to fill this gap, we propose a new simulation framework. Our approach, an R Implementation of a Transgenerational Hologenomic Model-based Simulator (RITHMS) is an open-source package. It builds upon simulated transgenerational genotypes from the Modular Breeding Program Simulator (MoBPS) package and incorporates distinctive characteristics of the microbiota, notably vertical and horizontal transmission as well as modulation due to the environment and host genetics. In addition, RITHMS can account for a variety of selection strategies and is adaptable to different genetic architectures. We simulated transgenerational hologenomic data using RITHMS under a wide variety of scenarios, varying heritability, microbiability, and microbiota transmissibility. We found that simulated data accurately preserved key characteristics across generations, notably microbial diversity metrics, exhibited the expected behavior in terms of correlation between taxa and of modulation of vertical and horizontal transmission, response to environmental effects and the evolution of phenotypic values depending on selection strategy. Our results support the relevance of our simulation framework and illustrate its possible use for building a selection index balancing genetic gain and microbial diversity and for evaluating the impact of partially observed microbiota data. RITHMS is an advanced, flexible tool for generating transgenerational hologenomes under selection that incorporate the complex interplay between genetics, microbiota and environment.

==> PCJ-pagedegarde.tex <==
\makeatletter
\newgeometry{margin=2.54cm,top=2.54cm}
\thispagestyle{empty}

% --- Badge en overlay (hors flux) ---
\begin{tikzpicture}[remember picture,overlay]
  \node[anchor=north east,xshift=-15pt,yshift=-15pt]
    at (current page.north east)
    {\href{https://doi.org/10.24072/pci.mcb.100417}{%
      \includegraphics[height=35mm]{badge_PCI_Math_Comp_Biol.png}}};
\end{tikzpicture}
% -----------------------------------

\vfill

\ifx\PDGauthors\undefined\let\PDGauthors\authors\fi

\begin{minipage}[t]{.9\textwidth}
  \normalsize\setlength{\parskip}{3ex}
  \def\IsEqualContrib{\textsuperscript{$\#$,}\global\cdr@hasequalcontribtrue}

  {\raggedright\Huge\bf\@title\par}

  {\raggedright\LARGE\let\footnotesize=\normalsize\cdr@listauthors@footnotes\par}

  {\Large\url@sfstyle\printDOI}

  \bigskip{\huge\bf Abstract}\\[1ex]
  \normalsize{\setlength{\parskip}{0ex}\@abstract\par}

  \ifx\@empty\@keywords\else\textbf{Keywords:} \@keywords\par\fi

  \footnotesize\cdr@listaddresses@footnotes
  \ifcdr@hasequalcontrib,\quad\textsuperscript{$\#$}Equal contribution\par\fi

  \normalsize\textbf{Correspondence}\\
  {\url@sfstyle\url{\thePCIcorresp}}

\end{minipage}

\vfill
\restoregeometry

